Bayesian Methodologies with pyhf

bayesian_pyhf is a Python package that allows for the parallel Bayesian and frequentist evaluation of multi-channel binned statistical models. The Python library pyhf is used to build such models according to the HistFactory framework and already includes many frequentist inference methodologies. The pyhf-built models are then used as data-generating model for Bayesian inference and evaluated with the Python library PyMC. Based on Monte Carlo Chain Methods, PyMC allows for Bayesian modelling and together with the arviz library offers a wide range of Bayesian analysis tools.

==> Makefile <==
FILENAME = ms

date = $(shell date +%Y-%m-%d)
output_file = draft_$(date).pdf

figure_src = $(wildcard figures/*.tex figures/*/*.tex)
figure_list = $(figure_src:.tex=.pdf)

LATEX = lualatex

BIBTEX = bibtex

default: document copy_draft

all: default

figures: $(figure_list)

figures/%.pdf: figures/%.tex
	latexmk -$(LATEX) -interaction=nonstopmode -halt-on-error $(basename $@)
	mv $(notdir $(basename $@)).pdf $(basename $@).pdf
	rm $(notdir $(basename $@)).*

text:
	latexmk -$(LATEX) -logfilewarnings -halt-on-error -shell-escape $(FILENAME)

document: figures text

copy_draft:
	rsync $(FILENAME).pdf $(output_file)

clean:
	rm -f *.aux *.bbl *.blg *.dvi *.idx *.lof *.log *.lot *.toc \
		*.xdy *.nav *.out *.snm *.vrb *.mp \
		*.synctex.gz *.brf *.fls *.fdb_latexmk \
		*.glg *.gls *.glo *.ist *.alg *.acr *.acn *.pyg

clean_figures:
	rm -f $(figure_list)

clean_drafts:
	rm -f draft_*.pdf

realclean: clean clean_figures
	rm -f *.ps *.pdf

lint:
	grep -E --color=always -r -i --include=\*.tex --include=\*.bib "(\b[a-zA-Z]+) \1\b" || true

final:
	if [ -f *.aux ]; then \
		$(MAKE) clean; \
	fi
	$(MAKE) figures
	$(MAKE) abstract
	$(MAKE) text
	$(MAKE) clean
	$(MAKE) lint

arXiv: deep_clean text
	
	sed -i.bak 's/cache=false/cache=true/' latex/packages.tex
	$(MAKE) text

	mkdir submit_to_arXiv
	cp $(FILENAME).tex submit_to_arXiv
	if [ -f $(FILENAME).bbl ]; then cp $(FILENAME).bbl submit_to_arXiv/ms.bbl; fi
	cp Makefile submit_to_arXiv

	if [ -d src ]; then cp -r src submit_to_arXiv; fi
	if [ -d latex ]; then cp -r latex submit_to_arXiv; fi
	if [ -d figures ]; then cp -r figures submit_to_arXiv; fi
	if [ -f *.sty ]; then cp *.sty submit_to_arXiv; fi
	
	if [ -f *.bst ]; then cp *.bst submit_to_arXiv; fi
	
	if [ -f 00README.XXX ]; then cp 00README.XXX submit_to_arXiv; fi

	
	
	mv _minted-$(FILENAME) submit_to_arXiv/_minted-ms
	sed -i.bak 's/finalizecache/frozencache/' submit_to_arXiv/latex/packages.tex

	mv submit_to_arXiv/$(FILENAME).tex submit_to_arXiv/ms.tex

	
	
	sed -i.bak '/^ *

	
	
	

	find submit_to_arXiv/ -name "*.bak" -type f -delete

	
	find submit_to_arXiv/ -name "*.bib" -type f -delete

	tar -zcvf submit_to_arXiv.tar.gz submit_to_arXiv/
	rm -rf submit_to_arXiv
	$(MAKE) realclean

	
	if [ -f latex/packages.tex.bak ];then \
		mv latex/packages.tex.bak latex/packages.tex; \
	fi

list_arXiv:
	tar -tvf submit_to_arXiv.tar.gz

test_arXiv:
	tar -xzvf submit_to_arXiv.tar.gz
	cd submit_to_arXiv && make

clean_arXiv:
	if [ -f submit_to_arXiv.tar.gz ];then \
		rm submit_to_arXiv.tar.gz; \
	fi

deep_clean: realclean clean_arXiv
	rm -rf submit_to_arXiv


==> latex/packages.tex <==
\usepackage[varg]{txfonts}   % Web of Conferences font
\usepackage{amsmath,bm}
\usepackage{hyperref}
\graphicspath{{figures/}}
\usepackage{listings}
\RequirePackage{caption}
\RequirePackage{subcaption}  % Needed for subfigures
\usepackage[cache=true,newfloat=true,frozencache]{minted}
\usepackage[capitalize]{cleveref}% https://ctan.org/pkg/cleveref % Must be loaded after hyperref
\usepackage{lineno}
\usepackage{lmodern}% https://www.ctan.org/pkg/lm % Use same fonts as journal submission and match layout

\usemintedstyle{friendly}
\setminted[python]{}

\hypersetup{bookmarksnumbered=true, bookmarksopen=true, bookmarksopenlevel=0}
\hypersetup{pdftitle={Bayesian Methodologies with pyhf}, pdfauthor={Matthew Feickert, Lukas Heinrich, Malin Horstman}}
\hypersetup{colorlinks,breaklinks}
\hypersetup{linkcolor=blue,citecolor=blue,filecolor=black,urlcolor=blue}

